WeaQA: Weak Supervision via Captions for Visual Question Answering

Methodologies for training visual question answering (VQA) models assume the availability of datasets with human-annotated \textit{Image-Question-Answer} (I-Q-A) triplets. This has led to heavy reliance on datasets and a lack of generalization to new types of questions and scenes. Linguistic priors along with biases and errors due to annotator subjectivity have been shown to percolate into VQA models trained on such samples. We study whether models can be trained without any human-annotated Q-A pairs, but only with images and their associated textual descriptions or captions. We present a method to train models with synthetic Q-A pairs generated procedurally from captions. Additionally, we demonstrate the efficacy of spatial-pyramid image patches as a simple but effective alternative to dense and costly object bounding box annotations used in existing VQA models. Our experiments on three VQA benchmarks demonstrate the efficacy of this weakly-supervised approach, especially on the VQA-CP challenge, which tests performance under changing linguistic priors.

==> tables/supp_table_old.tex <==
% \begin{table*}[t]
%     \centering
%     \resizebox{\textwidth}{!}
% {
%     \begin{tabular}{l>{\raggedright}p{50mm}>{\raggedright}p{25mm}>{\raggedright}p{50mm}p{25mm}}
%         \toprule
%         \textbf{Mutation} & $\mathbf{Q}$ & $\mathbf{A}$ & $\mathbf{Q_{new}}$ & $\mathbf{A_{new}}$ \\
%         \toprule
%         \multirow{4}{*}{Negation} & Is this bread? & yes & Is this not bread & no \\
%          & What is the color of the woman's shirt? & black & What is not the color of the woman's shirt? & white\\
%          & Are there deciduous trees? & no & Are there no deciduous trees? & yes \\
%          & Is there a boy? & no & Is there no boy? & yes \\
%         \midrule
%         \multirow{3}{*}{Adversarial} & Who is riding the boat? & man & Who is riding the desk & \textit{``can't say"}\\
%          & How big is the plane? & large & How big is the book? & \textit{``size"} \\
%          & How many pillows are on the bed? & four & How many pillows are on the table? & \textit{``number"} \\
        % \midrule 
        % \multirow{4}{*}{Paraphrasing} & How is something parked ? & illegally & How's-what's parked? & illegally\\
        %  & what does something seem to do ? & park & What do you think something seems to be doing? & park\\
        %  & Where was parked something? & behind a legally parked car & Do you know where something was parked? & behind a legally parked car \\
        %  & How many cars are visible ? & 2 & How many cars are we looking at? & 2 \\
        %  & Is there two cars parked on the sidewalk on the street ? & Yes & There are two cars parked on the sidewalk, right? & Yes \\
        %  & Is it a bathroom sink with toiletries on the counter ? & Yes & Is a washbasin with toiletries on counter? & Yes \\
        %  \midrule
        %   \multirow{4}{*}{Templates} & What are set on the sidewalk outside a veterinary hospital? & bags &  & \\
        %  & What is the young man holding up in front of his face ? & phone &  & \\
        %  & What is almost empty on the table & glass &  & \\
        %  & What drawn carriage with passengers in the city & horse &  &  \\
        %  & What is the color of the table ? & white &  &  \\
        %  & What is the color of the eyes ? & blue &  &  \\
        % %  & How many boats anchored by ropes close to shore? & 8 & & \\
    %     \bottomrule
    % \end{tabular}
    % }
    % \caption{Examples of three types of question transformation with corresponding answers}
    % \label{tab:negation}

% \end{table*}


